Super-approximation, I: p-adic semisimple case

Let $k$ be a number field, $\Omega$ be a finite symmetric subset of $\mathbb{GL}_{n_0}(k)$, and $\Gamma=\langle \Omega\rangle$. Let \[ C(\Gamma):=\{\mathfrak{p}\in V_f(k)|\hspace{1mm} \Gamma \text{is a bounded subgroup of} \mathbb{GL}_{n_0}(k_{\mathfrak{p}})\}, \] and $\Gamma_{\mathfrak{p}}$ be the closure of $\Gamma$ in $\mathbb{GL}_{n_0}(k_{\mathfrak{p}})$. Assuming that the Zariski-closure of $\Gamma$ is semisimple, we prove that the family of left translation actions $\{\Gamma\curvearrowright \Gamma_{\mathfrak{p}}\}_{\mathfrak{p}\in C(\Gamma)}$ has {\em uniform spectral gap}. As a corollary we get that the left translation action $\Gamma\curvearrowright G$ has {\em local spectral gap} if $\Gamma$ is a countable dense subgroup of a semisimple $p$-adic analytic group $G$ and Ad$(\Gamma)$ consists of matrices with algebraic entries in some $\mathbb{Q}_p$-basis of Lie$(G)$. This can be viewed as a (stronger) $p$-adic version of \cite[Theorem A]{BISG}, which enables us to give applications to the Banach-Ruziewicz problem and orbit equivalence rigidity.

==> SG_EscapeModQ.tex <==
\subsection{}\label{ss:EscapeModQ}
The main goal of this section is to prove escape from proper subgroups of $\pi_Q(\Gamma)$ where $Q=p^n$ is a power of a prime $p$.
\begin{prop}\label{p:EscapeModQ}
Let $\Omega$ be as in Proposition~\ref{p:EscapeSubgroups}. Then there is a positive number $\delta$ (depending on $\Omega$) such that for any $n\gg_{\Omega} 1$ and any proper subgroup $H$ of $\pi_{p^n}(\Gamma)$ we have
\[ 
\pcal_{\pi_{p^n}(\Omega)}^{(l)}(H)\le [\pi_{p^n}(\Gamma):H]^{-\delta},
\]
for $l\ge \frac{n}{\delta}\log p$.
\end{prop} 
We start with a (well-known) lemma which gives us the Frattini subgroup of the congruence subgroups of $\gcal(\bbz_p)$, where (as before) $\gcal$ is the closure of $\bbg$ in $(\mathcal{GL}_{N_0})_{\bbz_S}$. Let $G(p^m):=\{g\in \gcal(\bbz_p)|\h \pi_{p^m}(g)=1\}$. This kind of result for semisimple groups and large $p$ goes back to Weisfeiler~\cite{Wei}.
\begin{lem}\label{l:Frattini}
Let $\gcal$ and $G(p^m)$ be as above. If $m_0\ge 2$, $\wt{H}$ be a closed subgroup of $G(p^{m_0})$ and $\wt{H}G(p^{m_0+1})=G(p^{m_0})$, then $\wt{H}=G(p^{m_0})$. And so the Frattini subgroup $\Phi(G(p^{m_0}))=G(p^{m_0+1})$.
\end{lem} 
\begin{proof}
By induction on $k$ we prove  that $\wt{H}G(m_0+k)=G(m_0)$. The base of the induction is given by the assumption. To get the induction step, it is enough to prove that $(\wt{H}\cap G(m_0+k))G(m_0+k+1)=G(m_0+k)$. By Lemma~\ref{l:PropertiesOfLinearizationMap}, we have $\lin{p^{m_0}}{p^{m_0+1}}:G(p^{m_0})/G(p^{m_0+1})\rightarrow \gfr/p\gfr$ is an isomorphism. And so by the assumption, for any $x\in \gfr$ there is $h\in \wt{H}$ such that $\pi_{p^{m_0+1}}(h)=\pi_{p^{m_0+1}}(I+p^{m_0}x)$. On the other hand, if $m_0\ge 2$, then $\pi_p(((I+p^{m_0}x')^p-I)/p^{m_0+1})=\pi_p(x')$. And so $\linValue{p^{m_0+k}}{p^{m_0+k+1}}{h^{p^k}}=\pi_p(x)$, which, by Lemma~\ref{l:PropertiesOfLinearizationMap}, implies the induction step. Since $\wt{H}$ is a closed subgroup, we have that $\wt{H}=G(p^{m_0})$.
\end{proof}  
The following lemma is the adjoint representation version of \cite[Corollary 14]{SGV}. 
\begin{lem}\label{l:ProjSSPart}
Let $\bbg$ be as before and $\hfr\subset \ugfr(\bbq_p)$ be a proper $\bbg(\bbq_p)$-invariant subspace. Then the projection of $\hfr$ to the semisimple part $\ugfr_{s}(\bbq_p)$ of $\ugfr(\bbq_p)$ is a proper subspace.
\end{lem}
\begin{proof}
Suppose to the contrary that $\hfr$ maps onto $\ugfr_s(\bbq_p)$. We can identify $\ugfr(\bbq_p)$ with $\ugfr_s(\bbq_p)\oplus \bbv(\bbq_p)$ as an $\bbg_s(\bbq_p)$-module, where $\bbg_s(\bbq_p)$ acts on $\ugfr_s(\bbq_p)$ via the adjoint action and on $\bbv(\bbq_p)$ via the given representation. Since $\ugfr(\bbq_p)$ is a completely reducible $\bbg_s(\bbq_p)$-module, there are a $\bbg_s(\bbq_p)$-module homomorphism
\[
\theta: \ugfr_s(\bbq_p) \rightarrow \bbv(\bbq_p),
\] 
and a proper $\bbg_s(\bbq_p)$-submodule $V'\subset \bbv(\bbq_p)$ such that 
\be\label{e:Submodule}
\hfr=\{(x,\theta(x)|\h x\in \ugfr_s(\bbq_p)\}\oplus V'.
\ee
Since $\bbv(\bbq_p)$ acts trivially on $\ugfr(\bbq_p)/\bbv(\bbq_p)$ and graph of $\theta$ is $\bbv(\bbq_p)$-invariant, $\bbv(\bbq_p)$ acts trivially on the graph of $\theta$. On the other hand, $\bbv(\bbq_p)$ is abelian and $\ugfr(\bbq_p)$ is the sum of the graph of $\theta$ and $\bbv(\bbq_p)$. Hence $\bbv(\bbq_p)$ acts trivially on $\ugfr(\bbq_p)$ which implies that $\bbv\subseteq Z(\bbg)$. This contradicts our assumption that $\bbg$ is perfect. 
\end{proof}
\begin{lem}\label{l:SmallLifts}
Let $\gcal$ and $G(p^m)$ be as before. Then there is a positive number $\delta$ such that for any prime $p\not\in S$ and an open subgroup $\wt{H}$ of $G(p^2)$ the set
\[
\lcal_{\delta}(\wt{H}):=\{\lambda\in \gcal(\bbz_S)\cap \wt{H}|\h \|\lambda\|_S\le [\gcal(\bbz_p):\wt{H}]^{\delta}\}
\]
is in a proper Zariski-closed subgroup of $\bbg$.
\end{lem}
\begin{proof}
Let $l(\wt{H}):=\min\{k\in \bbz^+|\h \wt{H}\supseteq G(p^k)\}$.  
Notice that since $H$ is an open subgroup, $l(\wt{H})$ is finite. By Lemma~\ref{l:Frattini}, we have that $(\wt{H}\cap G(p^k)) G(p^{k+1})/G(p^{k+1})$ is a proper $\f_p$-subspace of $G(p^k)/G(p^{k+1})\simeq \gfr/p\gfr$. Thus we have 
\be\label{e:LevelIndex}
p^{l(\wt{H})-2}\le [G(p^2):\wt{H}] \le p^{d (l(\wt{H})-2)},
\ee
where $d=\dim_{\f_p}\gfr/p\gfr$. Now let 
\[
\overline{V}_{\wt{H}}:=\lin{p^{l'}}{p^{l}}((\wt{H}\cap G(p^{l'}))G(p^l)/G(p^l))\subseteq \gfr/p^{l-l'}\gfr,
\]
 where $l:=l(\wt{H})$ and $l':=\lceil l/2\rceil$. So there are a $\bbz_p$-basis $\ebf_1,\ldots,\ebf_d$ of $\underline{\gfr}(\bbz_p)$ and positive integers $n_1\le \cdots 
 \le n_{d'}$ such that $\overline{W}_{\wt{H}}=\pi_{p^l}(\sum_{i=1}^{d'} p^{n_i} \bbz_p \ebf_i)$ (for some $d'\le d$). Since
 \[
 0=n_0\le n_1\le \cdots \le n_{d'} \le \lfloor l/2 \rfloor=: n_{d'+1},
 \]
 there is $i_0$ such that $n_{i_0}-n_{i_0-1}=\Theta_d(l)$. Let $W_{\wt{H}}:=\sum_{i=1}^{i_0-1} p^{n_i} \bbz_p \ebf_i\subset \underline{\gfr}(\bbz_p)$ (if $i_0=1$, then $W_{\wt{H}}=0$). So $\pi_{p^{n_{i_0}}}(W_{\wt{H}})$ is $H$-invariant under the adjoint action. 
 
If $W_{\wt{H}}$ is $\gcal(\bbz_p)$-invariant, then by Lemma~\ref{l:ProjSSPart} the projection $W_s$ of $\underline{W_{\wt{H}}}(\bbq_p)$ to the semisimple part $\ugfr_s(\bbq_p)$ of $\ugfr(\bbq_p)$ is not onto. Since $\ugfr_s(\bbq_p)$ is a completely reducible $\bbg_s(\bbq_p)$-module and the simple factors are the Lie algebras of the simple factors of $\bbg_s$, there is $M\subset \ugfr_s(\bbz_p)$ with the following properties:
\begin{enumerate}
	\item $M$ is a primitive $\bbz_p$-submodule of $\ugfr(\bbz_p)$ (i.e. its $\bbz_p$-basis can be extended to a $\bbz_p$-basis of $\ugfr(\bbz_p))$. 
	\item $[W_s,M]=0$.
	\item $W_s\cap M=0$.
\end{enumerate}   
Let $x\in M\setminus pM$ (since $M$ is primitive, this condition is equivalent to $\|x\|_p=1$).  Let $h\in \wt{H}$ and suppose $h\in G(p^k)\setminus G(p^{k+1})$ for some $k\le \lceil l/2\rceil$. Then there is $y\in W_s$ such that $p^{-k}\log h\in y+p^{n_{i_0}-\lceil l/2\rceil}\ugfr(\bbz_p)+\bbv(\bbq_p)$. And so 
\[
\ad(\log h)(x)\in p^{\Theta_d(l)}\ugfr_s(\bbz_p)\oplus (\bbv(\bbq_p) \cap p^2 \ugfr(\bbz_p)).
\]
and so
\[
\Ad(h)(x)=\exp(\ad(\log h))(x)\in x+p^{\Theta_d(l)}\ugfr_s(\bbz_p)+ \bbv(\bbq_p).
\]
Now consider the action of $\gcal(\bbz_p)$ on $\overline{\ugfr_s(\bbz_p)}:=\ugfr(\bbz_p)/(\bbv(\bbq_p)\cap \ugfr(\bbz_p))$. And let $\overline{W}_{wt{H}}$ be the projection of $\bbz_p x+W_{\wt{H}}$ to $\overline{\ugfr_s(\bbz_p)}$. So by the above discussion, $\pi_{p^{\Theta_d(l)}}(\overline{W}_{\wt{H}})$ is $\wt{H}$-invariant but not $\gcal(\bbz_p)$-invariant.

It is well-known (for instance by reduction theory) that $\gcal(\bbz_S)$ is a finitely generated group. We fix a finite generating set $\Omega'$ of $\bbg(\bbz_S)$.

So altogether we have that there are $c(d)<1<C(d)$ such that 
for some $w\in \ugfr(\bbz_p)$ and $l\in \ugfr^*(\bbz_p):=\hom_{\bbz_p}(\ugfr(\bbz_p),\bbz_p)$ the following holds
	\begin{enumerate}
	\item for any $h\in \wt{H}$,  $|l(\Ad(h)(w))|_p\le [\gcal(\bbz_p):\wt{H}]^{-c}$;
	\item for some $\gamma\in \Omega'$, $|l(\Ad(\gamma)(w))|_p\ge [\gcal(\bbz_p):\wt{H}]^{-c/C}$,
  \end{enumerate}
  
Let $\eta_g(x,y):=y(\Ad(g)(x))$ for $(x,y)\in \ugfr(R)\times \ugfr^*(R)$ and $g\in \gcal(R)$ and $\bbz_S$-algebra $R$. We claim that if $\delta$ is small enough, there is $(x,y)\in (\ugfr\times\ugfr^*)(\overline{\bbq})$ such that
\begin{enumerate}
	\item For any $h\in \lcal_{\delta}(\wt{H})$ we have $\eta_h(x,y)=0$,
	\item For some $\gamma\in \Omega'$ we have $\eta_{\gamma}(x,y)\neq 0$. 
\end{enumerate}
This implies that $\lcal_{\delta}(\wt{H})$ is in a proper subvariety of $\bbg$. Now (as in~\cite{EMO}) using the generalized Bezout theorem we have that the group generated by $\lcal_{\Theta_{\dim \bbg}(\delta)}(\wt{H})$ is not Zariski-dense in $\bbg$. 

 We notice that the above implies that there is $(x_0,y_0)\in (\ugfr\times\ugfr^*)(\bbz_p)$ such that
\begin{enumerate}
	\item For any $h\in \lcal_{\delta}(\wt{H})$ we have $|\eta_h(x_0,y_0)|_p\le [\gcal(\bbz_p):\wt{H}]^{-(1-1/C)c}$,
	\item For some $\gamma \in \Omega'$ we have $\eta_{\gamma}(x_0,y_0)=p^{\Theta_{\Omega'}(1)}$.
\end{enumerate}

To prove the above claim, we proceed by contradiction and use an effective version of Nullstellensatz theorem~\cite{BY} (as in~\cite{BG1}). To be precise, we assume that the following has no solution over $\overline{\bbq}$:
\[
\forall\h h\in \lcal_{\delta}(\wt{H}),\h \eta_h(x,y)=0,\h \eta_{\gamma}(x,y)=p^{n_0},
\]
where $\gamma\in \Omega'$ and $n_0=\Theta_{\Omega'}(1)$ are the ones given above. So by the effective Nullstellensatz, e.g.~\cite{BY}, there are polynomials $q_{\gamma}, q_h\in \bbz_S[\ugfr\times \ugfr^*]$ and $D_0\in \bbz_S$ such that 
\[
 q_{\gamma}(x,y)(\eta_{\gamma}(x,y)-p^{n_0})+\sum_{h\in \lcal_{\delta}(\wt{H})} q_h(x,y) \eta_h(x,y)=D_0,
\]
and
$\|D_0\|_S\le [\gcal(\bbz_p):\wt{H}]^{\Theta(\delta)}$. After plugging in $x_0$ and $y_0$ we get a contradiction if $\delta$ is small enough. 
\end{proof}
\begin{proof}[Proof of Proposition~\ref{p:EscapeModQ}]
By strong approximation~\cite{Nor} we know that $[\gcal(\bbz_p):\overline{\Gamma}]\ll_{\Gamma} 1$, where $\overline{\Gamma}$ is the closure of $\Gamma$ in $\gcal(\bbz_p)$. For a proper subgroup $H$ of $\pi_{p^n}(\Gamma)$, let $\wt{H}:=\{h\in \gcal(\bbz_p)|\h \pi_{p^n}(h)\in H\}$. So by Lemma~\ref{l:SmallLifts} we have that $\lcal_{\delta_1}(\wt{H})$ is in a proper algebraic subgroup $\bbh$ of $\bbg$ for small enough $\delta_1$. So by Proposition~\ref{p:EscapeSubgroups} we have that
\be\label{e:EscapeModQ}
\pcal^{(l)}(\{\gamma\in \Gamma|\h \pi_{p^n}(\gamma)\in H\})\le e^{-\delta_0 l}
\ee
if $1\ll l\ll \delta_1\log [\pi_{p^n}(\Gamma):H]$ where $\delta_0$ is given by Proposition~\ref{p:EscapeSubgroups} and $\delta_1$ is given by Lemma~\ref{l:SmallLifts}.

If for some $l\ge \frac{n}{\delta}\log p$ we have $\pcal_{\pi_{p^n}(\Omega)}^{(l)}(H)\ge [\pi_{p^n}(\Gamma):H]^{-\delta}$, then  by Lemma~\ref{l:BGRemark} for any $l'\le \frac{n}{\delta}\log p$ we have  $\pcal_{\pi_{p^n}(\Omega)}^{(2l')}(H)\ge [\pi_{p^n}(\Gamma):H]^{-2\delta}$. This contradicts (\ref{e:EscapeModQ}) if $\delta$ is small enough.
\end{proof}

==> SG_NecessaryNori.tex <==
\subsection{Necessity.}\label{ss:Necessity} Let us just remark that proof of~\cite[Section 5.1]{SGV} can be adjusted to give the necessary part of Theorem~\ref{t:main}.
The only difference is that the proof in \cite{SGV} makes use of the fact that the congruence kernels modulo square-free numbers define a topology, but here we need a result which works for any infinite sequence of positive integers. All the given arguments are well-known and they are included for the  convenience of the reader. 

\begin{lem}\label{l:FiniteIndexSubgroup}
Let $\Gamma$ be a finitely generated group generated by a symmetric set $\Omega$, and $\Lambda$ be a finite index normal subgroup of $\Gamma$. Let $\{N_i\}$ be a family of finite index normal subgroups of $\Gamma$. Then $\Gamma$ has property($\tau$) with respect to $\{N_i\}$ if and only if $\Lambda$ has property($\tau$) with respect to $\{N_i\cap \Lambda\}$. (See~\cite[Chapter 4.3]{Lub})
\end{lem}
\begin{proof}
Suppose $S=\{s_1,\ldots,s_k\}$ is a symmetric generating set of $\Gamma$ and at the same time $\Gamma=\bigcup_{i=1}^k s_i\Lambda$. So for any $1\le i,j\le k$ there is $1\le l=l(i,j)\le k$ such that $s_l\Lambda=s_is_j\Lambda$. Let $s'_{i,j}:=s_{l(i,j)}^{-1}s_is_j\in \Lambda$. Then we claim that $\Lambda$ is generated by $S':=\{s'_{i,j}\}\cup (S\cap \Lambda)$. Let $\Lambda_1$ be the group generated by $S'$. Clearly it is a subgroup of $\Lambda$. By the definition of $s'_{i,j}$ we have that $s_{l(i,j)}\Lambda_1=s_is_j\Lambda_1$. And so $\Gamma=\bigcup_{i=1}^k s_i\Lambda_1$ since $S$ generates $\Gamma$ and is symmetric. Therefore we get that $\Lambda_1=\Lambda$.  

Assume that $\Gamma$ has property($\tau$) with respect to $\{N_i\}$. So there is $\vare>0$ such that for any $i$ and any unit vector $u$ of
\[
l^2_0(\Gamma/N_i):=\{f:\Gamma/N_i\rightarrow \bbc|\h \sum_{\bar{\gamma}\in \Gamma/N_i} f(\bar{\gamma})=0\},
\]
we have
\be\label{e:NotAlmostInvariant}
\max_{s_i\in S}\{\|s_i u-u\|\}>\vare.
\ee
Now assume that $v$ is a unit vector in an irreducible non-trivial representation $\rho:\Lambda/(N_i\cap \Lambda)\rightarrow \GL(V)$ which is an $\vare'$-almost invariant vector with respect to $S'$, i.e. for any $s'\in S'$ we have
\[
\|\rho(s')(v)-v\|<\vare'. 
\]
By Frobenius reciprocity, $\tilde\rho:={\rm Ind}_{\Lambda/(N_i\cap \Lambda)}^{\Gamma/N_i}\rho$ is a subrepresentation of $l^2_0(\Gamma/N_i)$. Let $\{s_{i'}\}_{i'\in I}\subseteq S$ be a set which induces (distinct) coset representatives of $\Lambda N_i/N_i$ in $\Gamma/N_i$.  Then $\tilde\rho$ can be described as follows: $W:=\bigoplus_{i'\in I}s_{i'}V$ (where $s_{i'}V$ are orthogonal copies of $V$) and, for any $\gamma\in \Gamma$, we have 
\[
\tilde\rho(\gamma)(\sum_{i'\in I} s_{i'}x_{i'})=\sum_{i'\in I}s_{l'_{\gamma}(i')}\rho(s_{l'_{\gamma}(i')}^{-1}\gamma s_{i'})(x_{i'}),
\]
where $l'_{\gamma}(i')$ is the unique element of $I$ such that $s_{l'_{\gamma}(i)}\Lambda N_i=\gamma s_{i'}\Lambda N_i$. 

Notice that for any $i',j$ we have $s_{l'_{s_{i'}}(j)}^{-1}s_{i'}s_{j}$ is a multiple of at most 5 elements of $S'$, and so we have
\[
\|\rho(s_{l'_{s_{i'}}(j)}^{-1}s_{i'}s_{j})(v)-v\|<5\vare'.
\]
Hence, for any $1\le i'\le k$, we have
\begin{align*}
\|\tilde\rho(s_{i'})(\sum_{j\in I} s_j v)-\sum_{j\in I} s_j v\|&=
\|\sum_{j\in I}s_{l'_{s_{i'}}(j)}\rho(s_{l'_{s_{i'}}(j)}^{-1}s_{i'}s_{j})(v)-\sum_{j\in I} s_j v\|\\
&\le 5|\Gamma/\Lambda|\vare'+\|\sum_{j\in I}s_{l'_{s_{i'}}(j)}v-\sum_{j\in I} s_j v\|=5|\Gamma/\Lambda|\vare'.
\end{align*}
So by (\ref{e:NotAlmostInvariant}) we have that 
$
\vare< 5|\Gamma/\Lambda|\vare'.
$
Thus no non-trivial irreducible representation of $\Lambda/(N_i\cap \Lambda)$ has an $\vare/(5|\Gamma/\Lambda|)$-almost invariant vector with respect to $S'$, which proves that $\Lambda$ has property($\tau$) with respect to $\{N_i\cap \Lambda\}$. 

Now assume that $\Lambda$ has property($\tau$) with respect to ${N_i\cap \Lambda}$. So there is $\vare>0$ such that for any unit vector $u\in l^2_0(\Lambda/(\Lambda\cap N_i))$ we have
\be\label{e:NotAlmostInvariant2}
\max_{s'\in S'}\|s'u-u\|>\vare. 
\ee
Let $\rho$ be an irreducible representation of $\Gamma/N_i$ which does not factor through $\Gamma/\Lambda$. Suppose that $v$ is a unit vector in $V_{\rho}$ which is $\vare'$-almost invariant vector with respect to $S$, i.e.
\[
\|\rho(s)(v)-v\|\le \vare',
\]
for any $s\in S$. Therefore for any $s'\in S'$ we have
\[
\|\rho(s')(v)-v\|\le 3\vare'.
\]
By Frobenius reciprocity and, since $\rho$ does not factor through $\Gamma/\Lambda$, the restriction of $\rho$ to $\Lambda/(\Lambda \cap N_i)$ is a subrepresentation of $l^2_0(\Lambda/(\Lambda \cap N_i))$. Thus by (\ref{e:NotAlmostInvariant2}) we have $\vare<3 \vare'$, which implies that any non-trivial representation of $\Gamma/N_i$ has no $\vare''$-almost invariant vector with respect to $S$ for some $0<\vare''<\vare/3$. 
\end{proof}
\begin{cor}\label{c:FiniteIndexSubgroup}
Let $\Gamma$ be a finitely generated group and $\Omega$ be a symmetric finite generating set of $\Gamma$. Assume $\Lambda$ be a finite-index subgroup of $\Gamma$. Then $\Lambda$ has a finite symmetric generating set $\Omega'$, and for any infinite set $\{N_i\}$ of normal finite index subgroups of $\Gamma$,  $\{\Cay(\Gamma/N_i,\pi_{N_i}(\Omega))\}_i$ is a family of expanders if and only if $\{\Cay(\Lambda/(N_i\cap \Lambda),\pi_{N_i\cap \Lambda}(\Omega'))\}_i$ is a family of expanders.
\end{cor}
\begin{proof}
This is a direct corollary of Lemma~\ref{l:FiniteIndexSubgroup} and \cite[Theorem 4.3.2]{Lub}.
\end{proof}
\begin{lem}~\label{l:Necessary}
Let $\Omega$ be a finite symmetric subset of $\GL_n(\bbz[1/q_0])$ and  $\Gamma=\langle \Omega\rangle\subseteq \GL_n(\bbz[1/q_0])$. Let $\bbg^{\circ}$ be the Zariski-connected component of the Zariski-closure $\bbg$ of $\Gamma$ in $(\mathbb{GL}_n)_{\bbq}$. If $\{\Cay(\pi_{q_i}(\Gamma),\pi_{q_i}(\Omega))\}_i$ is a family of expanders for integers $q_1<q_2< \cdots$ coprime with $q_0$, then $\bbg^{\circ}$ is perfect, i.e. $[\bbg^{\circ},\bbg^{\circ}]=\bbg^{\circ}$. 
\end{lem} 
\begin{proof}
Let $\Gamma^{\circ}:=\Gamma\cap \bbg^{\circ}$. Then, by Corollary~\ref{c:FiniteIndexSubgroup}, $\Gamma^{\circ}$ has a finite symmetric generating set $\Omega^{\circ}$ and 
\[
\{\Cay(\pi_{q_i}(\Gamma^{\circ}),\pi_{q_i}(\Omega^{\circ}))\}_i
\]
is a family of expanders. Therefore for some positive integer $C$ we have $|\pi_{q_i}(\Gamma^{\circ})/[\pi_{q_i}(\Gamma^{\circ}),\pi_{q_i}(\Gamma^{\circ})]|<C$ for any $i$.

On the other hand, $\bbg^{\circ}$ and $[\bbg^{\circ},\bbg^{\circ}]$ are $\bbq$-groups, and the quotient map $\bbg^{\circ}\xrightarrow{f} \bbg^{\circ}/[\bbg^{\circ},\bbg^{\circ}]$ is a $\bbq$-homomorphism. Therefore $\bbg^{\circ}/[\bbg^{\circ},\bbg^{\circ}]$ can be viewed as a $\bbq$-subgroup of $\mathbb{GL}_{n'}$ such that first the quotient map $f$ induces a $\bbq$-homomorphism from $\bbg$ to $\mathbb{GL}_{n'}$ and second $f(\Gamma^{\circ})\subseteq \GL_{n'}(\bbz[1/q_0])$. So there is an integer $q'$ such that for any prime $p$ we have $\|f(\gamma)-I\|_p\le |q'|_p^{-1} \|\gamma-I\|_p$. Therefore $f$ induces an onto homomorphism from $\pi_{q_i}(\Gamma^{\circ})/[\pi_{q_i}(\Gamma^{\circ}),\pi_{q_i}(\Gamma^{\circ})]$ onto $\pi_{q_i/\gcd(q_i,q')}(f(\Gamma^{\circ}))$. Hence for any $i$ we have
\[
|\pi_{q_i/\gcd(q_i,q')}(f(\Gamma^{\circ}))|<C.
\]
Since $f(\Gamma^{\circ})$ is a Zariski-dense subset of $\bbg^{\circ}/[\bbg^{\circ},\bbg^{\circ}]$ and modulo arbitrarily large integers it has at most $C$ elements, we have that $\bbg^{\circ}/[\bbg^{\circ},\bbg^{\circ}]$ is finite. So by the connectedness we have that $\bbg^{\circ}$ is perfect.
\end{proof}
In the rest of this article we deal with the sufficiency part. And so from this point on we assume that the connected component $\bbg^{\circ}$ of the Zariski-closure of $\Gamma=\langle \Omega\rangle$ is perfect (unless otherwise is mentioned). 
